A Streamwise GAN Vocoder for Wideband Speech Coding at Very Low Bit Rate

Recently, GAN vocoders have seen rapid progress in speech synthesis, starting to outperform autoregressive models in perceptual quality with much higher generation speed. However, autoregressive vocoders are still the common choice for neural generation of speech signals coded at very low bit rates. In this paper, we present a GAN vocoder which is able to generate wideband speech waveforms from parameters coded at 1.6 kbit/s. The proposed model is a modified version of the StyleMelGAN vocoder that can run in frame-by-frame manner, making it suitable for streaming applications. The experimental results show that the proposed model significantly outperforms prior autoregressive vocoders like LPCNet for very low bit rate speech coding, with computational complexity of about 5 GMACs, providing a new state of the art in this domain. Moreover, this streamwise adversarial vocoder delivers quality competitive to advanced speech codecs such as EVS at 5.9 kbit/s on clean speech, which motivates further usage of feed-forward fully-convolutional models for low bit rate speech coding.

==> Makefile <==
####################################################################################
# Latex Makefile
#
# Compilation of files written in LaTeX (version 0.5)
#
# Initial Author : Sebastien Varrette <Sebastien.Varrette@imag.fr>
# Edited by Guillaume Fuchs
#
# --------------------------------------------------------------------------------
# This is a generic makefile in the sense that it doesn't require to be 
# modified when adding/removing new source files.
# --------------------------------------------------------------------------------
#
# Documentation on the Makefile utility may be found at 
#                  http://www.gnu.org/software/make/manual/make.html           
# 
# Traditionaly, the command 'latex f.tex' generates the following files :
#     - f.dvi
#     - f.aux
#     - f.log
#     - f.bbl in case of bibliography references 
#     - etc...
# When running make,
# DVI, PDF and Postscript files will be located in the $(OUTPUT_DIR) directory 
# whereas all other files generated will move to $(TRASH_DIR)/. 
#
# Available Commands  
# ------------------
# make       : Compile LaTeX files, PDF/ps generated are placed in $(OUTPUT_DIR)/ 
# make force : Force re-compilation, even if not needed 
# make clean : Remove all generated files 
# make html  : generate HTML files from tex in $(HTML_DIR)/ (using latex2html)
#                  The directory is created on the first invocation
# make help      : print help message 
#
############################## Variables Declarations ##############################
# Directory where PDF, Postcript files and other generated files will be placed
OUTPUT_DIR = Output
TRASH_DIR  = .Trash
HTML_DIR   = $(OUTPUT_DIR)/HTML
# Check avalibility of source files
TEX_SRC    = $(subst ./,,$(shell find . -maxdepth 1 -name "*.tex" | xargs echo))
ifeq ($(TEX_SRC),)
all:
	@echo "No source files available - I can't handle the compilation"
	@echo "Please check the presence of source files (with .tex extension)"
else
# Main tex file and figures it may depend on 
MAIN_TEX   = $(shell grep -l "[\]begin{document}" $(TEX_SRC) | xargs echo)
FIGURES    = $(shell find . -name "*.eps" -o -name "*.png" | xargs echo)
ifeq ($(MAIN_TEX),)
all:
	@echo "I can't find any .tex file with a '\begin{document}' directive "\
		"among $(TEX_SRC). Please define a main tex file!"
else
# Commands used during compilation
LATEX      = $(shell which latex)
LATEX2HTML = $(shell which latex2html)
BIBTEX     = $(shell which bibtex)
DVIPS      = $(shell which dvips)
DVIPDF     = $(shell which dvipdf)
LATEXPDF   = $(shell which latexpdf)
PSPDF      = $(shell which ps2pdf)
GZIP       = $(shell which gzip)
PDFLATEX   = $(shell which pdflatex)
# Generated files
DVI    	     = $(MAIN_TEX:%.tex=%.dvi)
PS           = $(MAIN_TEX:%.tex=%.ps)
PS_GZ        = $(MAIN_TEX:%.tex=%.ps.gz)
PDF          = $(MAIN_TEX:%.tex=%.pdf)
OUTPUT_DVI   = $(DVI:%=$(OUTPUT_DIR)/%)
OUTPUT_PS    = $(PS:%=$(OUTPUT_DIR)/%)
OUTPUT_PDF   = $(PDF:%=$(OUTPUT_DIR)/%)
BACKUP_FILES = $(shell find . -name "*~")
# Files to move to $(TRASH_DIR) after compilation
# Never add *.tex (or any reference to source files) for this variable.
TO_MOVE      = *.aux *.log *.toc *.lof *.lot *.bbl *.blg 

############################### Now starting rules ################################
# Required rule : what's to be done each time 
all: $(OUTPUT_PDF)

# Dvi files generation
$(OUTPUT_DVI) $(DVI): $(TEX_SRC) $(FIGURES)
	@echo "==> Now generating $(OUTPUT_DVI)"
	@for f in $(MAIN_TEX); do                                         \
	 	$(LATEX) $$f;                                             \
		bib=`grep "^[\]bibliography{" $$f|sed -e "s/^[\]bibliography{\(.*\)}/\1/"|tr "," " "`;\
		if [ ! -z "$$bib" ]; then                                 \
		  	echo "==> Now running BibTeX ($$bib used in $$f)";\
			$(BIBTEX) `basename $$f .tex`;                    \
			$(LATEX) $$f;                                     \
		fi;                                                       \
	 	$(LATEX) $$f;                                             \
		trash=`ls $(TO_MOVE)2>/dev/null|xargs echo`;              \
		if [ ! -z "$$trash" -a -d $(TRASH_DIR) ]; then            \
			echo "==> Now moving $$trash to $(TRASH_DIR)/";   \
			mv -f --target-directory=$(TRASH_DIR)/ $$trash;   \
		fi;                                                       \
	done                                                      
	@if [ ! -d $(OUTPUT_DIR) ]; then                           \
			echo "$(OUTPUT_DIR)/ does not exist";             \
			echo "==> Now creating $(OUTPUT_DIR)/";           \
			mkdir -p ./$(OUTPUT_DIR);                         \
	fi                                                       
	@mv $(DVI) $(OUTPUT_DIR)/ 	   	                         
	@echo "$(OUTPUT_DVI) generated"                          

# Postscript generation
$(OUTPUT_PS) $(PS): $(OUTPUT_DVI)
	@echo "==> Now generating $(OUTPUT_PS)"
	@for dvi in $(OUTPUT_DVI); do                                            \
		ps=`basename $$dvi .dvi`.ps;                              \
		$(DVIPS) -t a4 -Ppdf -q -o $$ps $$dvi;                                \
		mv $$ps $(OUTPUT_DIR)/;                                     \
	done

# PDF generation
$(OUTPUT_PDF) $(PDF) : $(OUTPUT_PS)
	@echo "==> Now generating $(OUTPUT_PDF)"
	@for ps in $(OUTPUT_PS); do                                            \
		pdf=`basename $$ps .ps`.pdf;                            \
		$(PSPDF) $$ps $$pdf;                                          \
		mv $$pdf $(OUTPUT_DIR)/;                                    \
	done

# PDF generation by forcing fonts to be embedded
embedpdf : $(OUTPUT_PDF) 
	@echo "==> Now embedding $(OUTPUT_PDF)"
	@for pdf in $(OUTPUT_PDF); do                                            \
		epdf=`basename $$pdf .pdf`_embedded.pdf;                            \
		gs -dNOPAUSE -dNOCACHE -dBATCH -sDEVICE=pdfwrite -dSubsetFonts=false -dEmbedAllFonts=true -dPDFSETTINGS=/prepress -sOutputFile=$$epdf $$pdf;       \
		mv $$epdf $(OUTPUT_DIR)/;        \
	done



pdflatex: $(TEX_SRC) $(FIGURES)
	@echo "==> Now generating $(OUTPUT_PDF)"
	@for f in $(MAIN_TEX); do                                         \
	 	$(PDFLATEX) $$f;                                             \
		bib=`grep "^[\]bibliography{" $$f|sed -e "s/^[\]bibliography{\(.*\)}/\1/"|tr "," " "`;\
		if [ ! -z "$$bib" ]; then                                 \
		  	echo "==> Now running BibTeX ($$bib used in $$f)";\
			$(BIBTEX) `basename $$f .tex`;                    \
			$(PDFLATEX) $$f;                                     \
		fi;                                                       \
	 	$(PDFLATEX) $$f;                                             \
		trash=`ls $(TO_MOVE)2>/dev/null|xargs echo`;              \
		if [ ! -z "$$trash" -a -d $(TRASH_DIR) ]; then            \
			echo "==> Now moving $$trash to $(TRASH_DIR)/";   \
			mv -f --target-directory=$(TRASH_DIR)/ $$trash;   \
		fi;                                                       \
	done                                                      
	@if [ ! -d $(OUTPUT_DIR) ]; then                           \
			echo "$(OUTPUT_DIR)/ does not exist";             \
			echo "==> Now creating $(OUTPUT_DIR)/";           \
			mkdir -p ./$(OUTPUT_DIR);                         \
	fi                                                       
	@mv $(PDF) $(OUTPUT_DIR)/ 	   	                         
	@echo "$(OUTPUT_PDF) generated"    
	

# Clean option
clean:
	rm -f *.dvi $(TO_MOVE) $(BACKUP_FILES)
	@if [ ! -z "$(OUTPUT_DIR)" -a -d $(OUTPUT_DIR) ]; then            \
                for f in $(MAIN_TEX); do                                  \
                        base=`basename $$f .tex`;                         \
                        echo "==> Now cleaning $(OUTPUT_DIR)/$$base*";    \
                        rm -rf $(OUTPUT_DIR)/$$base*;                     \
                done                                                      \
	fi
	@if [ ! -z "$(TRASH_DIR)" -a -d $(TRASH_DIR) ];   then            \
		for f in $(MAIN_TEX); do                                  \
			base=`basename $$f .tex`;                         \
			echo "==> Now cleaning $(TRASH_DIR)/$$base*";     \
			rm -rf $(TRASH_DIR)/$$base*;                      \
		done                                                      \
	fi
	@if [ ! -z "$(HTML_DIR)" -a -d $(HTML_DIR) ];     then            \
		echo "==> Now removing $(HTML_DIR)";                      \
		rm  -rf $(HTML_DIR);                                      \
	fi

# force recompilation
force :
	@touch $(MAIN_TEX)
	@$(MAKE)

# Test values of variables - for debug purpose  
test:
	@echo "--- Directories --- "
	@echo "OUTPUT_DIR -> $(OUTPUT_DIR)"
	@echo "TRASH_DIR  -> $(TRASH_DIR)"
	@echo "HTML_DIR   -> $(HTML_DIR)"
	@echo "--- Compilation commands --- "
	@echo "LATEX      -> $(LATEX)"
	@echo "PDFLATEX   -> $(PDFLATEX)"
	@echo "LATEX2HTML -> $(LATEX2HTML)"
	@echo "BIBTEX     -> $(BIBTEX)"
	@echo "DVIPS      -> $(DVIPS)"
	@echo "DVIPDF     -> $(DVIPDF)"
	@echo "GZIP       -> $(GZIP)"
	@echo "--- Files --- "
	@echo "TEX_SRC    -> $(TEX_SRC)"
	@echo "MAIN_TEX   -> $(MAIN_TEX)"
	@echo "FIGURES    -> $(FIGURES)"
	@echo "BIB_FILES  -> $(BIB_FILES)"
	@echo "DVI        -> $(DVI)"
	@echo "PS         -> $(PS)"
	@echo "PS_GZ      -> $(PS_GZ)"
	@echo "PDF        -> $(PDF)"
	@echo "TO_MOVE    -> $(TO_MOVE)"
	@echo "OUTPUT_PS_GZ -> $(OUTPUT_PS_GZ)"
	@echo "OUTPUT_PDF   -> $(OUTPUT_PDF)"
	@echo "BACKUP_FILES -> $(BACKUP_FILES)"

# print help message
help :
	@echo '+-----------------------------------------------------------------+'
	@echo '|                      Available Commands                         |'
	@echo '+---------------+-------------------------------------------------+'
	@echo '| make          | Compile LaTeX files.                            |'
	@echo '|               |   DVI/PS/PDF generated are placed in $(OUTPUT_DIR)/ |'
	@echo '| make pdflatex | Compile LaTeX files with pdflatex.              |'
	@echo '|               |   PDF generated is placed in $(OUTPUT_DIR)/     |'
	@echo '| make embedpdf | Embed fonts of teh pdf file in $(OUTPUT_DIR)/   |'
	@echo '| make force    | Force re-compilation, even if not needed        |'
	@echo '| make clean    | Remove all generated files                      |'
	@echo '| make html     | Generate HTML files from TeX in $(HTML_DIR)/    |'
	@echo '| make help     | Print help message                              |'
	@echo '+---------------+-------------------------------------------------+'


# HTML pages generation using latex2html
# First check that $(LATEX2HTML) and $(HTML_DIR)/ exist
html :
ifeq ($(LATEX2HTML),)
	@echo "Please install latex2html to use this option!"
	@echo "('apt-get install latex2html' under Debian)"
else
	@if [ ! -d ./$(HTML_DIR) ]; then                                         \
		echo "$(HTML_DIR)/ does not exist => Now creating $(HTML_DIR)/"; \
		mkdir -p ./$(HTML_DIR);                                         \
	fi
	-cp --target-directory=. $(TRASH_DIR)/*.aux $(TRASH_DIR)/*.bbl
	$(LATEX2HTML) -show_section_numbers -local_icons -split +1 \
		-dir $(HTML_DIR) $(MAIN_TEX)
	@rm -f *.aux *.bbl $(HTML_DIR)/*.tex $(HTML_DIR)/*.aux $(HTML_DIR)/*.bbl
	@echo "==> HTML files generated in $(HTML_DIR)/" 
	@echo "May be you can try to execute 'mozilla ./$(HTML_DIR)/index.html'"
endif
endif
endif

